Robust Performance Analysis of Source-Seeking Dynamics with Integral Quadratic Constraints

We analyze the performance of source-seeking dynamics involving either a single vehicle or multiple flocking-vehicles embedded in an underlying strongly convex scalar field with gradient based forcing terms. For multiple vehicles under flocking dynamics embedded in quadratic fields, we show that the dynamics of the center of mass are equivalent to the dynamics of a single agent. We leverage the recently developed framework of $\alpha$-integral quadratic constraints (IQCs) to obtain convergence rate estimates. We first present a derivation of \textit{hard} Zames-Falb (ZF) $\alpha$-IQCs involving general non-causal multipliers based on purely time-domain arguments and show that a parameterization of the ZF multiplier, suggested in the literature for the standard version of the ZF IQCs, can be adapted to the $\alpha$-IQCs setting to obtain quasi-convex programs for estimating convergence rates. Owing to the time-domain arguments, we can seamlessly extend these results to linear parameter varying (LPV) vehicles possibly opening the doors to non-linear vehicle models with quasi-LPV representations. We illustrate the theoretical results on a linear time invariant (LTI) model of a quadrotor, a non-minimum phase LTI plant and two LPV examples which show a clear benefit of using general non-causal dynamic multipliers to drastically reduce conservatism.

==> doc/applications.tex <==
\section{Applications}
\subsection{Single quadrotor in a scalar field}
\subsection{Multiple quadrotors flocking towards the source}


==> theorems/proof_Theorem_perf_analysis.tex <==
\begin{proof}[Theorem \ref{theom:theorem_perf_analysis}]
Since $\left[\begin{array}{c|c}
\mathcal{A}     &  \mathcal{B}\\
\hline
\mathcal{C}     &  \mathcal{D}
\end{array}\right]$ represents the state-space representation of $\Psi \begin{bmatrix}
G\\
I
\end{bmatrix}$,
let $\xi=\begin{bmatrix}
\Tilde{\eta} \\
x_{\psi}
\end{bmatrix}$ be the concatenation of the state $\Tilde{\eta}$ of $G$ (see \eqref{eq:sys_dyn_G_tilde}) and the filter state $x_{\Psi}$.
Consider the state-space representation
\begin{equation} \label{eq:sys_dyn_psi_GI}
    \begin{split}
        \Dot{\xi}&=\mathcal{A}\xi + \mathcal{B}\Tilde{u} \quad\quad \xi(0)=[\Tilde{\eta}_0^T \quad \mathbf{0}]^T\\
        \Tilde{z}&=\mathcal{C}\xi + \mathcal{D}\Tilde{u}
    \end{split}
\end{equation}
and observe that the output $\Tilde{z}$ of \eqref{eq:sys_dyn_psi_GI} is the one defined in \eqref{eq:signal_defn_z} with $\Tilde{y}$ defined as the output of $G$ for input $\Tilde{u}$, i.e., 
\begin{equation}\label{eq:signal_defn_y}
    \Tilde{y}(t)=\int_0^t C_{G} e^{A_{G}(t-\tau)}B_{G}\Tilde{u}(\tau)d\tau.
\end{equation}
Furthermore, dynamics \eqref{eq:sys_dyn_G} ensures that $\Tilde{u},\Tilde{y}$ satisfy \eqref{eq:delta}. 
Hence, Theorem \ref{theom:theorem_LMI_ZF} implies
\begin{equation} \label{eq:zPz_pos}
    \int_0^T e^{2\alpha t}\Tilde{z}^T(t) (P \otimes I_d) \Tilde{z}(t) dt \geq 0 \quad \forall P \in \mathbb{P},\forall T \geq 0.
\end{equation}

Define a storage function $V(\xi)=\xi^T \mathcal{X} \xi$.
Using \eqref{eq:perf_LMI} and dynamics \eqref{eq:sys_dyn_psi_GI}, we get,
\begin{equation*}
\begin{split}
\frac{d}{dt}(V(\xi(t)))+2\alpha V(\xi(t))
    &=\begin{bmatrix}
    \xi & \Tilde{u}
    \end{bmatrix}
    \begin{bmatrix}
    \mathcal{A}^T\mathcal{X}+\mathcal{X}\mathcal{A}+2\alpha \mathcal{X}  & \mathcal{X}\mathcal{B} \\
    \mathcal{B}^T\mathcal{X}    & \mathbf{0}
    \end{bmatrix}
    \begin{bmatrix}
    \xi\\ \Tilde{u}
    \end{bmatrix}\\ 
    &\leq
    -\begin{bmatrix}
    \xi & \Tilde{u}
    \end{bmatrix}
    \begin{bmatrix}
\mathcal{C}^T \\
\mathcal{D}^T 
\end{bmatrix}
( P\otimes I_d)
\begin{bmatrix}
\mathcal{C} & \mathcal{D} 
\end{bmatrix}
\begin{bmatrix}
    \xi\\ \Tilde{u}
    \end{bmatrix}\\
    &=-\Tilde{z}^T(t) (P \otimes I_d) \Tilde{z}(t)   
\end{split}.
\end{equation*}
Rearranging and integrating from $0$ to $T$, we obtain,
\begin{equation*}\label{eq:diff_diss_ineq}
\begin{split}
\frac{d}{dt}(e^{2\alpha t}V(\xi(t))) + e^{2\alpha t}\Tilde{z}^T(t) (P \otimes I_d) \Tilde{z}(t) &\leq 0\\
V(\xi(T)) + \int_0^T e^{2\alpha t}\Tilde{z}^T(t) (P \otimes I_d) \Tilde{z}(t) dt &\leq e^{-2\alpha t}V(\xi(0))
\end{split}
\end{equation*}
Using \eqref{eq:zPz_pos} and $\mathcal{X}>0$,
\begin{equation*}
    \begin{split}
        V(\xi(T)) &\leq e^{-2\alpha t}V(\xi(0))\\
        & \implies \\
        ||\xi|| &\leq \sqrt{\textnormal{cond}(\mathcal{X})} \cdot ||\xi(0)|| \cdot  e^{-\alpha t}\\
        & \implies \\
        ||\Tilde{\eta}|| &\leq \sqrt{\textnormal{cond}(\mathcal{X})} \cdot ||\xi(0)|| \cdot  e^{-\alpha t}\\
        & \implies \\
        ||\Tilde{y}|| &\leq ||C_G|| \cdot ||\Tilde{\eta}|| \\
        & \leq ||C_G|| \sqrt{\textnormal{cond}(\mathcal{X})} \cdot ||\xi(0)|| \cdot  e^{-\alpha t} \\
        &= \kappa e^{-\alpha t}
    \end{split}
\end{equation*}
\end{proof}
